ASH: Agents that Self-Hone in Long-Horizon Worlds

Long-horizon visuomotor tasks remain a fundamental challenge in AI, as current methods rely on hand-engineered rewards or action-labeled demonstrations, neither of which scales. We introduce ASH, an agentic system that learns a long-horizon policy from unlabeled, noisy internet video, without reward shaping or expert annotation. ASH follows a self-improvement loop; when it gets stuck, ASH learns an Inverse Dynamics Model (IDM) from its own trajectories, and uses its IDM to extract supervision from relevant internet video. ASH uses unsupervised learning to identify key moments from large-scale internet video and retains them as long-term memory - allowing it to tackle long-horizon problems. We evaluate ASH on two complementary environments demanding multi-hour planning: Pokemon Emerald, a turn-based RPG, and The Legend of Zelda: The Minish Cap, a real-time action-adventure game. In both games, behavioral cloning, retrieval-augmented and zero-shot foundation-model baselines plateau, while ASH sustains progression across our 8-hour evaluation. ASH reaches an average of 11.2/12 milestones in Pokemon Emerald and 9.9/12 in Legend of Zelda, while the strongest baseline gets stuck in both environments at an average of 9.3/12 and 7.8/12 milestones, respectively. We demonstrate that self-improving agents are a scalable recipe for learning in long-horizon worlds. Our project page is https://toolbox-hq.github.io/ASH

==> algorithms/ash_v2.tex <==
\makeatletter


\begin{algorithm}[H]
\caption{\method}
\label{alg:ash_apx}
\begin{hyphenrules}{nohyphenation}
\algrenewcommand\alglinenumber[1]{\scriptsize #1:}

\begin{algorithmic}[1]
\setlength{\itemsep}{.25ex}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
\fontsize{8.5pt}{8pt}\selectfont
\Require Number of agents $N$, short-term memory length $\shortlen$, long-term memory length $\longlen$, max steps without new key moment $\Delta$, retrieval match length $\retlen$, number of videos retrieved $k$, internet dataset $\DI$

\Statex \textbf{Step 0: Initialization}
\State $\pi \gets \text{Initialize \method{} policy}$
\State $\mathcal{K} \gets \text{Initialize new key moment classifier}$
\State $\text{IDM} \gets \text{Initialize IDM}$
\State $\mathcal{E}_{\oneToN} \gets \text{Initialize environments}$ \Comment{All agents start at the beginning of the environment.}
\State ${\tau}_{\oneToN} \gets \emptyset$ \Comment{Per agent environment trajectories.}
\State $\mathcal{M}_{\oneToN} \gets \emptyset$ \Comment{Key moment memory per agent.}

\Statex \textbf{Step 1: Inference}
\State $\delta \gets 0$  \Comment{Steps since last retrieval.}
\State $C_{\oneToN} \gets 0$ \Comment{Per-agent stuck counters}
\While{$\max_n C_n < \Delta$}
\State $\delta \gets \delta + 1$
\For{$n=1$ to $N$}
  \State $\lmem \gets \mathcal{M}_{n,\,-\longlen:}$  \Comment{Retrieve \longlen{} most recent long-memories from the agent's memory bank.}
  \State $a \sim \pi\!\left(\cdot \mid \tau_{n,\,-\shortlen:},\, \lmem\right)$ \Comment{Predict action using short and long-term memory.}
  \State $o \gets \mathcal{E}_n(a)$
  \State $\tau_n \gets \tau_n \cup \{(o,a)\}$
  \If{$\mathcal{K}(\tau_n,\, |\tau_n|)$} \Comment{Add observation to memory bank if it is a \emph{new key moment}.}
    \State $\mathcal{M}_n \gets \mathcal{M}_n \cup \{o\}$
    \State $C_n \gets 0$ \Comment{Reset steps since last new key moment counter.} 
  \EndIf
  \State $C_n \gets C_n + 1$
\EndFor
\EndWhile
\Statex \textbf{Step 2: Retrieval}
\State $\mathcal{D}^{{R}} \gets \emptyset$
\For{$n=1$ to $N$}
    \State $\mQ \gets \Call{Embed}{\tau_{n,-\delta:}}$
    \State $\text{scores} \gets \emptyset$
    \For{$\tau^{\mathrm{obs}} \in \DI$}
        \State $\mE \gets \Call{Embed}{\tau^{\mathrm{obs}}}$ \Comment{$\mE$ is cached for efficiency.}
        \State $e \gets \Call{Rows}{\mE}$
        \State $\mS \gets \mQ \mE^\top$
        \State $z^\star \gets -\infty$
        \For{$t \in \{1, \ldots, e - \retlen + 1\}$} \Comment{Compute scores over windows.}
            \State $s \gets \mS_{:,\,t:t+\retlen}$
            \State $z \gets 0$
            \For{$j=1$ to $\retlen$}
                \State $r^\star \gets \arg\max_r s_{r,j}$
                \State $z \gets z + s_{r^\star,j}$
                \State $s_{r^\star,:} \gets -\infty$
            \EndFor
            \State $z^\star \gets \max(z^\star, z)$
        \EndFor
        \State $\text{scores} \gets \text{scores} \cup \{(\tau^{\mathrm{obs}}, z^\star)\}$
    \EndFor
    \State $\mathcal{D}^{{R}} \gets \mathcal{D}^{{R}} \cup \{\operatorname{top\text{-}k}(\text{scores})\}$ \Comment{Unionize videos into a dataset.}
\EndFor
\Statex \textbf{Step 3: Policy Bootstrapping}

\State Update $\mathcal{K}$ using $\DR$
\State Update IDM on $\tau_{\oneToN}$
\State $\Dpi \gets \emptyset$
\For{$\obs \in \DR$}
  \For{$t = 1$ to $|\obs| - \shortlen + 1$ step $\shortlen$}
    \State $\tilde{\mA} \gets \mathrm{IDM}(\obs_{t:t+\shortlen})$ \Comment{Use IDM to create pseudo-actions for internet data item.}
    \State $\bar{\lmem} \gets [\,\obs_i \,:\, i < t,\, \mathcal{K}(\obs, i)\,]$ \Comment{Find key moments in $\tau^{{obs}}$.}
    \State $\Dpi \gets \Dpi \cup \bigl\{\bigl(\obs_{t:t+\shortlen},\, \tilde{\mA},\, \bar{\lmem}_{-\longlen:}\bigr)\bigr\}$ \Comment{Add sample to dataset.}
  \EndFor
\EndFor
\State Update $\pi$ on $\Dpi$
\State \texttt{GoTo} \textbf{Step 1}

\end{algorithmic}

\end{hyphenrules}
\end{algorithm}

%\endgroup
\makeatother
